Re:Cognize -- A Framework For Open-Set Comic Character Re-Identification

Comics and manga tell stories through characters whose appearances change from panel to panel, yet readers recognise them hundreds of pages later without ever consulting a cast list. Character re-identification models rarely face the same challenge: existing evaluations give them a fixed set of identities before the story begins. \textbf{Re:Cognize} instead asks models to recognise characters as the story unfolds and learn who is who along the way. Across three manga corpora, we evaluate five Re-ID backbones and \textbf{MECHA}, a memory-augmented baseline we introduce, and find that the central difficulty lies somewhere unexpected. Recognising familiar characters is nearly solved. Knowing which matches to trust is not. When models build a gallery and grow it from their own predictions, their performance deteriorates, even though correct identity labels would improve it by over twenty points. This raises a simple question: when should a model trust its own match? We derive a single comparison that determines when gallery updates improve recognition and use it to design \textbf{VOUCH}, which updates its memory only when the page provides supporting evidence. Without fitting additional parameters, VOUCH recovers between one-third and two-thirds of the improvement available from perfect labels. RE:COGNIZE measures whether a model can recognise characters as it reads; VOUCH shows how to remember them reliably. We focus our methodological claims on identity maintenance for previously encountered characters, while separately evaluating new-character emergence as a diagnostic under a fixed reference rule to distinguish recognition from discovery.

==> tables/cross_corpus_summary.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.05}
\caption{\textbf{Transfer beyond \PopChars}, headline rows. Manga109 is 27 held-out volumes. \emph{Pretrained} is the released backbone with no \PopChars training at all. \emph{Finetuned} and \emph{$+$ Mem.} are \PopChars-trained checkpoints scored zero-shot here from one training run, the latter the \MeCha configuration with the highest P1 mAP on this corpus, so the first gap is what BNNeck fine-tuning on another corpus is worth and the second is \MeCha. P4 is identity Rank-1 at $k=1$ under random seeding at $B_{\max}=50$, for that same configuration. Re:Verse is one series (Re:Zero) and its two columns are the released backbone with no \PopChars training. Manga109 cells are the mean over three seed draws, Re:Verse cells over five. The full tables are Table~\ref{tab:manga109_results} and Table~\ref{tab:reverse_results} in the appendix. Three vision-language models on the same Re:Verse benchmark reach 1.11, 0.00 and 0.85 percent character-identification accuracy~\citep{baranwal2025reverse}.}
\label{tab:cross_corpus}
\begin{tabular}{l|ccc|c|cc}
\toprule
\rowcolor{gray!15}
& \multicolumn{4}{c|}{\textbf{Manga109}, 27 volumes} & \multicolumn{2}{c}{\textbf{Re:Verse}, 1 series, pretrained} \\
\rowcolor{gray!15}
& \multicolumn{3}{c|}{P1 mAP} & \textbf{P4 id.\ R-1} & \multicolumn{2}{c}{P1} \\
\rowcolor{gray!15}
\multirow{-3}{*}{\textbf{Backbone}} & \textbf{Pretrained} & \textbf{Finetuned} & \textbf{$+$ Mem.} & \textbf{$+$ Mem.} & \textbf{mAP} & \textbf{R-1} \\
\midrule
TransReID & 28.4 & 29.1 & 30.3 & 10.7 & 34.5 & 46.0 \\
MagiV2 & \textbf{65.3} & \textbf{65.9} & \textbf{67.4} & \textbf{47.1} & \textbf{84.2} & \textbf{91.0} \\
MagiV3 & 37.4 & 39.4 & 41.5 & 18.4 & 48.2 & 73.0 \\
InstructReID & 28.6 & 30.4 & 35.5 & 14.3 & 30.7 & 50.9 \\
ReID5o & 31.2 & 33.0 & 36.5 & 15.0 & 36.2 & 60.8 \\
\bottomrule
\end{tabular}
\end{table}

